ChEF: A Comprehensive Evaluation Framework for Standardized Assessment of Multimodal Large Language Models

Multimodal Large Language Models (MLLMs) have shown impressive abilities in interacting with visual content with myriad potential downstream tasks. However, even though a list of benchmarks has been proposed, the capabilities and limitations of MLLMs are still not comprehensively understood, due to a lack of a standardized and holistic evaluation framework. To this end, we present the first Comprehensive Evaluation Framework (ChEF) that can holistically profile each MLLM and fairly compare different MLLMs. First, we structure ChEF as four modular components, i.e., Scenario as scalable multimodal datasets, Instruction as flexible instruction retrieving formulae, Inferencer as reliable question answering strategies, and Metric as indicative task-specific score functions. Based on them, ChEF facilitates versatile evaluations in a standardized framework, and new evaluations can be built by designing new Recipes (systematic selection of these four components). Notably, current MLLM benchmarks can be readily summarized as recipes of ChEF. Second, we introduce 6 new recipes to quantify competent MLLMs' desired capabilities (or called desiderata, i.e., calibration, in-context learning, instruction following, language performance, hallucination, and robustness) as reliable agents that can perform real-world multimodal interactions. Third, we conduct a large-scale evaluation of 9 prominent MLLMs on 9 scenarios and 6 desiderata. Our evaluation summarized over 20 valuable observations concerning the generalizability of MLLMs across various scenarios and the composite capability of MLLMs required for multimodal interactions. We will publicly release all the detailed implementations for further analysis, as well as an easy-to-use modular toolkit for the integration of new recipes and models, so that ChEF can be a growing evaluation framework for the MLLM community.

==> math.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/2.Introduction.tex <==
\section{Introduction}
% Large language models (LLMs) have made significant advancements since the emergence of OpenAI's GPT series. ChatGPT and GPT-4~\citep{openai2023gpt4} have showcased impressive language generation capabilities, extensive knowledge, and reasoning abilities. By integrating visual information into LLMs, Multimodal Large Language Models (MLLMs) have demonstrated remarkable performance in visual question answering scenarios. Recent works, such as LLaVA~\citep{llava} and MiniGPT-4~\citep{minigpt4}, as well as InstructBlip~\citep{dai2023instructblip}, have highlighted the capabilities of these models in visual comprehension and reasoning. However, there is currently a lack of a standardized benchmark for evaluating the performance of MLLMs on traditional vision tasks. Given that MLLMs are generative models with free-form outputs, traditional evaluation methods are no longer suitable. Proposing a unified and reliable benchmark to assess these models poses a significant challenge.


% % 第一段只讲咋做，不说问题，然后提这些框架不一样，测出来结果不一样
% % 我们要做comprehensive framework，which is xxx。 有啥challenge，为啥comprehensive，讲清楚4个部分
% % 几个维度是不够的 holistic 
% Recently, considerable efforts have been made to develop benchmarks for evaluating LVLMs. Some studies~\citep{yin2023lamm,xu2023lvlmehub} assess the models' free-form output by employing language processing techniques or utilizing GPT models to gauge the correctness of the generated answers. However, the processing of language lacks reliability and the inclusion of GPT models tends to decrease efficiency and introduce subjectivity. Other approaches~\cite{liu2023mmbench,li2023seedbench,fu2023mme} have transformed visual question answering into a multiple-choice format, which restricts the model's output to options such as A/B/C/D or yes/no. While this type of evaluation is more objective and straightforward, it is not entirely reliable due to the following challenges:
% \begin{enumerate}
%     \item Certain LVLMs may not strictly adhere to the instruction of explicitly generating multiple-choice options in their responses. Models with less proficient \emph{instruction-following} capabilities may demonstrate lower accuracy on the assessed datasets. However, it is important to note that this does not necessarily indicate a weaker aptitude for handling specific tasks.
%     \item Most LVLMs suffer from \emph{hallucination} issues, where the options provided by the model may not be thoroughly considered or verified, but instead guessed. The accuracy of the model in multiple-choice tasks may not consistently reflect its performance in visual tasks.
%     \item The multiple-choice questions simplify the complexity of traditional visual tasks, such as object detection. Instead of requiring precise bounding boxes, they focus on inquiring about the direction of an object, such as up, down, left, or right.
%     \item Relying solely on the accuracy of a model in multiple-choice questions for evaluating its performance is inadequate. It is crucial to consider additional metrics that go beyond accuracy, like the effectiveness in real-world interactions with humans.
% \end{enumerate}
% Building upon these considerations, we present ChEF: a Comprehensive and Holistic Evaluation Framework for large vision language models. It facilitates unified and reliable evaluations, encompassing scalable traditional visual task datasets alongside existing multiple-choice datasets. The framework enables a holistic evaluation of the model's performance from various perspectives and angles, providing a comprehensive assessment of its capabilities. The framework comprises four key components: scenario, instruction, inferencer and metrics. 

% The \textbf{scenario} represents a specific task that necessitates evaluating the model's performance, encompassing datasets from various traditional visual tasks. In ChEF, scenarios are scalable, allowing the inclusion of any visual dataset. We have incorporated several prominent datasets, such as CIFAR, VOC2012, and also integrated recent multi-choice question answering datasets like MMBench~\citep{liu2023mmbench}.

% The \textbf{instruction} focuses on how to pose questions to the model, ensuring a reliable and desired output format. We designed various question formats, including providing different prompts or in-context examples tailored to specific scenarios. 

% The \textbf{inferencer} pertains to how the model answers questions. In addition to the traditional free-form output, we employ a probabilistic approach within a limited text scope to constrain the model's output. For each scenario, we have multiple methods to construct the scope. Furthermore, ChEF supports multi-turn question-answering as well as chain of thought (CoT) question answering, enabling the model to produce more reliable and desired output formats.

% The \textbf{metrics} are designed to evaluate the model's performance in various aspects, aiming to provide a comprehensive assessment of the model's quality beyond just accuracy, which serves as an umbrella term. To evaluate the model comprehensively from aspects such as reliability, interactivity, and robustness, ChEF includes an additional set of six necessary metrics: calibration, in-context learning, instruction following, language performance, hallucination, and robustness. The \emph{calibration} stage necessitates the model's aptitude in effectively conveying uncertainty within its predictions. \emph{In-context learning} evaluates the model's proficiency in emulating provided examples. \emph{Instruction following} scrutinizes the model's adherence to human instructions. \emph{Language performance} assesses the model's capability to generate responses that closely resemble human utterances. \emph{Robustness} metrics appraise the model's resilience against visual noise and textual perturbations. \emph{Hallucination} metrics gauge the model's reliability.

% In summary, our contributions can be summarized as follows:
% \begin{enumerate}
%     \item We developed a comprehensive and holistic evaluation framework for large vision language models, which facilitates evaluations across scalable scenarios, accommodating diverse instructions, inferencers, and metrics.
%     \item We have strategically formulated multiple instructions and inferencers tailored to specific scenarios, with the objective of augmenting the reliability of model outputs and enabling more precise performance evaluations.
%     \item We introduced six additional metrics to comprehensively evaluate the model's performance from various perspectives, providing a comprehensive assessment of the model's quality beyond accuracy alone.
% \end{enumerate}



Large language models (LLMs) have made significant advancements since the emergence of OpenAI's GPT series. ChatGPT and GPT-4~\citep{openai2023gpt4} have showcased impressive language generation capabilities, extensive knowledge, and reasoning abilities. By integrating visual information into LLMs, Multimodal Large Language Models (MLLMs) have demonstrated remarkable performance in visual question answering scenarios. Recent works, such as LLaVA~\citep{llava} and MiniGPT-4~\citep{minigpt4}, as well as InstructBlip~\citep{dai2023instructblip}, have highlighted the capabilities of these models in visual comprehension and reasoning. However, there is currently a lack of a standardized benchmark for evaluating the performance of MLLMs on traditional vision tasks. Given that MLLMs are generative models with free-form outputs, traditional evaluation methods are no longer suitable. Proposing a unified and reliable benchmark to assess these models poses a significant challenge.

Recently, considerable efforts have been made to develop benchmarks for evaluating MLLMs. Some studies~\citep{yin2023lamm,xu2023lvlmehub} have constructed multiple evaluation pipelines tailored to specific tasks, utilizing diverse criteria to assess performance. Certain studies~\cite{bitton2023visitbench, yu2023mmvet, shao2023tinylvlm} involve the utilization of GPT-4 to assess the correctness of the model's generated output. Other approaches~\cite{liu2023mmbench,li2023seedbench,fu2023mme} have constructed a multi-choice question-answering dataset for different vision tasks , which restricts the model's output to options such as A/B/C/D or yes/no, to provide a more objective and straightforward evaluation.

Traditional visual tasks exhibit a multitude of variations, with each task having its own distinct set of metrics. Even within the same task, different datasets and evaluation metrics are employed. The incorporation of MLLMs introduces the challenge of generating free-form outputs, resulting in each benchmark adopting its unique evaluation methodology with diverse criteria. Consequently, the evaluation results of a single model across different benchmarks can exhibit notable discrepancies. There is currently a lack of a unified framework for comparative analysis among these diverse evaluation criteria.

In this paper, our primary aim is to construct a framework capable of integrating a wide array of datasets and diverse evaluation criteria. This framework will facilitate comprehensive and standardized comparisons across various evaluation pipelines for each model. The establishment of this framework necessitates addressing the following inherent challenges:
\begin{enumerate}
    \item Certain MLLMs may not strictly adhere to the instructions of explicitly generating the desired output format in their responses, such as `(A)' for a multi-choice question. Models with less proficient \emph{instruction-following} capabilities may exhibit lower performance on the assessed datasets, leading to unfairness and unreliability.
    \item The conventional evaluation methodologies employed for traditional visual tasks are not applicable for assessing MLLMs. For instance, the BLEU score is unsuitable for evaluating image captioning due to the model's ability to generate responses with extensive contextual information, and expecting the model to accurately provide a bounding box in detection tasks is a formidable undertaking.
    \item Evaluating an MLLM model solely based on the matching rate between its generated answers and the reference answers is far from sufficient. Multiple intrinsic performance aspects necessitate consideration, including the notable \emph{hallucination} issue emphasized in  POPE~\citep{POPE}. Moreover, as an interactive conversational agent, the model's capacity to engage in meaningful interactions with humans holds paramount importance. It is imperative to incorporate metrics beyond accuracy to holistically assess the model's performance.
\end{enumerate}

facilitatesLeveraging these crucial considerations, we introduce ChEF: a Comprehensive and Holistic Evaluation Framework for Multimodal Large Language Models. This framework facilitates comprehensive evaluations by encompassing scalable datasets for visual tasks and different evaluation criteria, and employing diverse metrics that provide holistic assessments from various perspectives and angles. As shown in the left Figure~\ref{fig:overview}, in order to accommodate diverse query formats, varied model response approaches, and different evaluation methodologies across different datasets, ChEF is designed for the following four components: scenario, instruction, inferencer, and metrics.

The \textbf{scenario} represents datasets from various traditional visual tasks that necessitate evaluating the model's performance. In ChEF, scenarios are scalable, allowing the inclusion of any visual dataset. We have incorporated several prominent datasets, such as CIFAR10~\citep{cifar10} and VOC2012~\citep{pascal-voc-2012}, and recently published multi-choice question answering datasets like MMBench~\citep{liu2023mmbench}.

The \textbf{instruction} focuses on how to pose questions to the model. We designed various question formats, including providing different prompts or in-context examples tailored to specific scenarios. 

The \textbf{inferencer} pertains to how the model answers questions. In addition to the traditional free-form output, we employ PPL Inferencer, which is a probabilistic approach within a limited text scope to constrain the model's output. The text scope is specifically designed for each scenario. ChEF also supports multi-turn question-answering as well as chain of thought (CoT) question answering. 

The \textbf{metrics} are designed to evaluate the model's performance in various aspects, aiming to provide a holistic assessment of the model's quality beyond just accuracy. As shown in the right Figure~\ref{fig:overview}, ChEF includes an additional set of six necessary metrics: calibration, in-context learning, instruction following, language performance, hallucination, and robustness. The \emph{calibration} stage necessitates the model's aptitude in effectively conveying uncertainty within its predictions. \emph{In-context learning} evaluates the model's proficiency in emulating provided examples. \emph{Instruction following} scrutinizes the model's adherence to human instructions. \emph{Language performance} assesses the model's capability to generate responses that closely resemble human utterances. \emph{Robustness} metrics appraise the model's resilience against visual noise and textual perturbations. \emph{Hallucination} metrics gauge the model's reliability.

Our contributions can be summarized as follows:
\begin{enumerate}
    \item We developed a comprehensive and holistic evaluation framework for large vision language models, which facilitates evaluations across scalable scenarios, accommodating diverse instructions, inferencers, and metrics.
    \item We have strategically formulated multiple instructions and inferencers tailored to specific scenarios, with the objective of augmenting the reliability of model outputs and enabling more precise performance evaluations.
    \item We introduced six additional metrics to comprehensively evaluate the model's performance from various perspectives, providing a comprehensive assessment of the model's quality beyond accuracy alone.
\end{enumerate}

\begin{figure}[htb]
    \centering
    \includegraphics[width=\textwidth]{sections/Figs/comparison.pdf}
    \includegraphics[width=\textwidth]{sections/Figs/overview.pdf}
    \caption{\textbf{Overview of ChEF.} \textbf{Acc.} is the accuracy. \textbf{Acc.*} is the accuracy from GPT evaluation. \textbf{$\cap$} means overlap with ChEF.  \textbf{ICL} is In-context Learning. \textbf{Lang. Perf.} is Language Performance. \textbf{Instruct. Follow.} is Instruction Following. }
  \label{fig:overview}
\end{figure}

% 1）最开始讲llms背景，引出多模态（暗线逻辑是llm转为生成模型为主的评测，已经趋于成熟，mllm还方兴未艾），最后引出mllm的benchmark

% 2）简单review一下已有benchmark，可以概括为要么是做了个scenario，要么是尝试做了framework但没做好，导致目前社区缺少一个结果稳定合理的benchmark

% 3）引出我们做了个framework解决这个，接着开始讲做这件事情本身的challenge：mapping到framework的四个模块，scenario对应评价一个模型所需要的任务/domain等多样性；instruction对应prompt变化较大带来的模型结果变化极不稳定；inferencer对应生成式模型对于不同任务的评测，要通过拿到一段文本后和gt做对应来计算metric，如何对应是个挑战；metric对应评价模型的指标，只有acc远远不够，例如对于cv任务我们希望复用最贴近他的指标，对于gpt评测我们则需要想全新的metric。

% 4）引出我们framework的细节，四个模块分别代表什么，互相之间是什么关系：我们的framework允许user自行选择评测时的四个模块的setting，我们会提供default setting的结果，也会给出为什么这么选default setting的原因（隐含逻辑是mmbench类数据集的工作，只是我们的一个scenario，lvlmehub这种尝试做framework的工作，涉及到的setting也只是我们的子集，我们在同一个框架下和各scenario原有的工作做了对齐，保障大家能在一个合理框架下比较结果——进而，所有人都可以在这个framework上评测，也可以加scenario，甚至是instruction/inferencer/metric，我们做的是基于一个framework的生态工作，我们自己也会持续在这里补充），此处一个段落几句话讲清楚四个模块的含义，并且串联逻辑。**此段落强调comprehensive**

% 6）有了这个framework，我们也把四个模块的合理的setting都纳入进来了，很comprehensive，但我们发现，目前的评测在模糊评价模型的感知/推理能力和llm本身作为一个agent和人交互的holistic能力。引出holistic能力，我们参考nlp走得靠前的工作，在多模态上定义了六个维度的holistic能力，并且在我们的framework里对现有mllm做了评测。（两方面motivation，一是希望给出除perception reasoning外尽量独立的holistic能力的评测和观察；二是我们argue mllm要保留它作为agent可以通过接受图像模态并响应人的指令跟人交互的能力）通过例子讲清楚六个维度，针对这六个维度我们给了有价值的观察。

% 7）contribution：略


% 现有评测metric多样并且很难囊括所有vision task, 主要由于大语言模型输出#free-form#， 难以进行评测。现有的benchmark有的尝试使用GPT4来判断语言模型输出内容的正确与否(mmvet, visitbench, tiny-lvlm)，但是用llm来评判一个mllm输出内容的正确与否具有一定的misalignment；有的benchmark用一些nlp中的工具来提取生成的长文本中对任务问题的正面回答，但是这些自动化的工具无法覆盖到free-form中所有的情况，例如分类问题中的同义词、粗细粒度等；最近一些benchmark工作将一些视觉任务统一通过选择题的方式来评测(mmbench， MME， seedbench)，选择题评测的方式在当下最为直观，并且也更容易评测，但仍然存在一定的问题：
%     1. 有一些mllm不会follow 做选择题的instruction，来显示地在回答中给出选项，导致得到一个较低的准确率，这样的评测结果是不公平不可靠的，例如对于一个正确答案为a的样本，模型可能会说bcd都不是正确答案，而不说a是正确答案，在大部分benchmark工作中会评价为错
%     2. 模型有幻想问题，给出的选项未必是通过思考推理得到的，可能是猜的，例如模型认为选择题在绝大多数情况下的正确答案是c，那么对于任意一道题，它选c都会有相对较高的置信度，过高的bias则会导致幻想
%     3. 现有的选择题数据集在部分传统视觉任务上简化了难度，例如检测问题，问的是上下左右，而非传统定义的bbox，此外，对于细粒度类别分类以及caption任务仍然没有合理的评测方式。
%     % 4. 这些work都只给出了一个表象层面的数值结果，没有剖析评测的mllm在这些task branch上表现不好的foundamental ability。 % subject 需要想个名字， 垂直维度上的能力也要想个名字
%     4. 由于以上三点提到的模型输出free-form的问题以及幻想问题，仅仅使用accuracy来表现模型在特定scenario下的性能是不够的，一些metrics beyond accuracy 同样是mllm作为一个语言模型的societal considerations ， 
% expert —— holistic
% scenario —— metric
% 
% 因此我们提出了一个framework来对现有的mllm在所有传统的视觉任务数据集上或者其他所有benchmark提出的数据集上进行可靠的统一的评测，我们的framework主要针对以下三个问题：
%     1. 如何问问题。我们设计了不同的问问题的形式包括不同的prompt以及不同的问答例子(in-context example) 来让mllm尽可能地理解要做的任务以及我们期望得到的输出，从而让模型输出一个更加可靠的结果。
%     2. 模型如何回答问题。在囊括了free-form的回答形式之外，我们通过计算一定文本域内的概率使得模型的输出限制在一个范围内，对于选择题，这样的输出形式就是选项，对于常规的视觉任务，我们会构造一些其他可能回答的negative答案，限制模型的输出在给定的几句话的范围内。此外，我们还包含了chain of thought的问答以及多轮问答的回答问题方式。这些设计的目的是为了让模型输出一个我们想要的形式。
%     3. 如何判断模型的回答好坏。 对于open-form的回答形式，我们使用传统的方式进行评测，对于constraint的回答形式，我们统一采用准确率进行评测，从而能够最为简单直观地评价模型性能。
%  

% 基于这个framework，我们挑选了几个主流任务的数据集进行评测，并在现有的所有benchmark工作中提出的选择题数据集上进行评测，并设计了六种评测的configuration来，包括 calibration， hallucination， instruction following, in-context learning, language performance , corruptions
%     1. calibration： Calibration and appropriate expression of model uncertainty is especially critical for systems to be viable for deployment in high-stakes settings, including those where models inform decision-making——helm
%      具有好的校准性的模型， 其预测的confidence能充分表达它的准确率，即高的置信度直接表示很高的概率预测对，也能充分表达模型的不确定性，从而能够在风险场景下使用模型  ECE 
%     2. hallucination： 不要人云亦云
%     3. instruction following： 需要模型服从人为指令，听人话
%     4. icl： 能够模仿人给定的例子，输出desired output format and content
%     5. language performance: 能够说人话
%     6. corruptions: 能够抗扰动，包括图片模糊等噪声以及人输入的各种prompt。


% 现有benchmark的问题，现有benchmark主要关注点在三类：
%     1. 从数据层面去解决模型输出自由难以评测的问题，例如构造选择题(MMBench, SeedBench)、和判断题（MME），这类benchmark问题有：每个任务都有个分数，但为什么分低，举例子分低是因为什么维度不行
%         a. 选择题或判断问答的方式不仅仅考虑所谓的视觉理解能力或者视觉推理能力，也在测试模型的instruction following能力，更有指令遵从能力从而输出选项的模型往往会有更高的得分，并没有将能力维度独立出来 
%         b. 一些模型存在严重的幻想问题 POPE，所说的选项可能是猜的，尤其是判断题会容易说yes，尽管mmbench使用了circular eval来规避幻想问题，但是仍旧将理解理解推理能力与非幻象能力、抗扰动性能力混为一谈，没有独立开来。我们单独测了robustness, POPE
%         c. MMbench 采用gpt4来判断选项规避指令遵从问题，但是gpt4无法达到绝对精确的判断，尤其是对于那些输出长段的推理过程的模型。seedbench通过计算多个候选回答的likelihood来限制模型输出，但是存在calibration的问题。

%     2. 从评测方法上解决模型输出自动难以评测问题，例如使用一些文本处理操作（LAMM，lvlm）或者计算候选答案的likelihood来限制输出(lvlm,seedbench)或者gpt评测(mm-vet, visitbench)
%         a. 文本处理操作无法考虑到所有情况，例如分类中的同义词问题和粗细粒度问题，检测问题中的label-bbox align问题
%         b. metric问题，例如caption问题，输出的回答越长越细节，指标反而会低，现有metric未必合理。尽管选择题是一个相对合理的方式，但是选择题的问题前面也提到了
%         c. lvlm只在一个分类数据集imagenetvc上进行了计算likelihood的尝试，seedbench的问题前面提到
%         d. gpt评测问题前面提到

%     3. 定义评测不同维度的benchmark，大部分评测方式将任务定义为perception 和 reasoning两个大类，然后在大类里面定义小类，每个小类会从数据集中抽取部分子集作为测试集，但是这样的定义是不明确的，一些perception任务中存在推理过程，reasoning任务同样需要perception能力，两者无法独立。一些评测方式考虑到了其他的能力维度，例如POPE的hallucination，MMBench 的circular eval 实际在评测robustness
%         a. 对于视觉能力定义不明确，reasoning 与 perception 无法独立
%         b. 除了pope，没有对mllm其他能力维度的系统评测
%         c. 这些模型都没有评测涉及准确定位能力的任务，包括grounding和detection

% 水平科目能力想个名字
% 垂直本质能力想个名字
% variation 想场景，要6个维度都包含图

% 为此，我们希望解决以下几个问题：
%     1. 如何将一些非视觉能力维度与视觉能力维度独立
%     2. 如何定义视觉任务的能力维度，以及非视觉的能力维度，评测mllm作为一个agent的可交互性
%     3. 如何更加准确地评判模型在一些常规视觉任务上的性能 caption， detection， finegrained classification

% 因此我们提出
%     1. a benchmark framework， 包括 models,  icl retriever， different types of inferencer , negative option generator, metic。 
%         a. 包含不同的主流模型，包括常规的llava， instructblip，minigpt4这些，也包括输出special token的kosmos2（我们第一个进行kosmos2评测），如果加了bard，可以多一个api形式的model
%         b. icl retriever为icl能力的评测设计，同样可以像nlp一样作为一个未来的default评测方式，包含了多种不同的从数据集中选取不同数量的ice的方法。   给icl例子可以代替prompt 设计
%         c. inferencer 包含常规的generate生成，option constraints生成，带有cot的生成以及多轮问答的生成，对于主流的视觉数据集，我们都定义了一个相对合理的inferencer。 
%         d. negative option generator，针对option constraints inferencer 生成错误选项的方式，对于主流数据集给了一些例子
%         e. metric 对于不同pipeline定义了不同的metric，包括在常规generate方法下的常见metric，以及在option constraint下的acc metric
    
%     2. default settings， 我们给出了一些主流任务的主流数据集作为我们framework 可以评测的数据集的例子，并给出一个现阶段最为合理的setting,同时可以兼容现有的所有benchmark dataset
%         a. 分类任务用cifar10， inferencer 用option constraint， metric acc。能够规避同义词问题以及粗细粒度问题，并且相比现有的default genrate 方法，对于不同的prompt会产生更加稳定的数值结果
%         b. 细粒度分类 omnibenchmark，infernecer用多轮问答的option constraint， metric weightedacc。 首个在细粒度分类数据集上进行评测，能够同时评测分类准确性以及分类粒度
%         c. caption flickr, inferencer 用 option constraint， metric acc。首个尝试用option constraint评测long context generation，避免了bleu等不合理性
%         d. counting fsc147, inferencer用option constraint， metric acc。 评测模型精确的计数能力，并且将instruction following能力与计数能力独立（模型需要输出数字）
%         e. vqa scienceqa，inferencer用带有cot的option constraint， metric acc。将instruction following 能力独立
%         f. detection VOC2012， inferencer 用多轮option constraint， metric map，mar。首个直接评测检测性能的pipeline
%         g. 现有benchmark dataset：MME, MMBench， Seedbench，都使用option constraint。能够独立instruction following能力

%         % 存在问题的点：
%         % 1. 选择题用ppl并不能完全解决instruction following，有的模型能够在direct中回答出选项内容，但是选择题上会更高概率输出某一选项，例如喜欢说(A)，导致准确率下降
%         % 2. seedbench中calibration问题同样无法独立出去，calibration问题来源于ppl在不同token 长度的option下计算方式问题，由于后续token的条件概率会远高于第一个token的生成概率，因此越长token的答案通过平均后会概率更高，是由于第一个token的calibration很低，这一问题在cifar中会非常明显。seedbench和cifar中我们都加了answer template来总体提高第一个token的生成概率，能够降低calibration带来的影响，但是不能完全解决


%     3. 六个独立于视觉任务的能力维度
%         a. calibration : ece
%         b. hallucination: pope 不说胡话
%         c. instruction following： 前后匹配率
%         d. in-context learning： 性能维持率
%         e. language performance: gpt metric 
%         f. robustness： 性能维持率

% 我们的contribution 归纳为：
%     1. a framework ， 啥都兼容，并且有很多独特设计
%     2. 不定义视觉能力维度，而是每个dataset都可以评测，给了主流的例子，并且给了default setting， 评测方式相较之前更合理，独立出非视觉能力
%     3. 定义了6个非视觉能力，评测作为agent的交互性


==> sections/3.Related_Work.tex <==
% \section{Related Works}

% \subsection{MLLM}
% llava, mplug, minigpt4 ... 
% normal tokens, special tokens, performance on different tasks.  hard to evaluate because of free prediction

% our framework includes different types of mllm

% \subsection{Benchmarks that build a dataset}
% SEEDBench, MME, MMBench

% all these datasets are invovled in our framework

% change the format of open QA to multi-choice questions

% \subsection{Benchmarks that try different inferencer or metric}
% lvlm tried direct, ppl, multi-reasoning

% Seedbench use ppl for multi-choice questions constraint output

% lamm tried nltk tools for entity extraction

% mm-vet use gpt score eval

% visit bench use gpt rank eval

% mmbench and tiny lvlm used gpt to extract the answer from the prediction that can match the gt

% invovles different types of inferencer

% \subsection{Benchmarking capability}
% perception reasoning 
% POPE - hallucination
% MMBench - circular eval == consistency


% we evaluate six extra dimensions, including icl, calibration, robustness, instruction-following, hallucination, agent-interactive (GPT4)



% \subsection{nlp benchmarking capability}
\section{Related Works}

% \subsection{MLLM}
% llava, mplug, minigpt4 ... 
% normal tokens, special tokens, performance on different tasks.  hard to evaluate because of free prediction
\subsection{Multimodal Large Language Models}
Due to the success of large Language models (LLMs) like GPTs~\citep{radford2019language,brown2020language,ouyang2022training},  LLAMA~\citep{touvron2023llama} and Vicuna~\citep{chiang2023vicuna}, Multimodal Large Language Models (MLLMs) have recently experienced substantial development. InstructBLIP~\citep{dai2023instructblip}, LLaVA~\citep{llava}, and MiniGPT-4~\citep{minigpt4} are based on open-source LLMs using vision-language instruction tuning get promising results. mPLUG-Owl~\citep{ye2023mplugowl} leverages the capabilities of pre-trained LLMs, a visual knowledge module, and a connected visual abstractor module to effectively align images with text. LAMM~\citep{yin2023lamm} extend the research of MLLMs to point clouds and propose a training framework optimized for modalities' extension. Otter~\citep{li2023otter} utilizes multimodal context instruction tuning data, demonstrating an improved ability to follow instructions and in in-context learning. LLaMA-Adapter-v2~\citep{gao2023llamaadapterv2} propose an early fusion strategy to solve the interference between image-text alignment and instruction following learning targets.
Shikra ~\citep{chen2023shikra} and Kosmos-2~\citep{kosmos-2} integrate grounding data during the training phase, enabling the model to develop grounding capabilities. In order to comprehensively assess the capabilities of these MLLMs, we present the first Comprehensive Evaluation Framework (ChEF) that can holistically profile each MLLM and fairly compare different MLLMs.


\subsection{Benchmarks for Large Language Models}
% llm benchmarks的发展，已经较全面的测评了llm，引几篇llm benchmarks的工作，介绍helm 包括 CALIBRATION，iCl，Robustness等维度，介绍gpt作为测评指标合理性的几篇工作，
In recent years, significant efforts have been made to comprehensively evaluate large language models from diverse perspectives~\citep{liang2022helm,wang2023pandalm,bommasani2021opportunities,gehrmann2021gem,gehrmann2022gemv2,brown2020language,gao2021framework,von2022evaluate,srivastava2022beyond}.
\cite{gao2021framework} provides a unified framework to test autoregressive language models on a large number of different evaluation tasks.
\citet{liang2022helm} measures seven metrics that reflect a range of societal considerations, including accuracy, calibration, robustness, fairness, bias, toxicity, and efficiency, in order to improve the transparency of language models. \citet{li2023instructionfollowing} 
propose to evaluate the instruction following ability from the aspect of how well models can follow instructions that may not align with their priors. Recent studies evaluating the quality of natural language generation~\citep{zheng2023judging,liu2023geval,wang2023chatgpt} have indicated that GPT-based metrics typically exhibit superior performance compared to traditional reference-based and reference-free baseline metrics in terms of their correlation with human quality judgments. These evaluation metrics effectively assess the capabilities of LLMs from multiple dimensions. However, in the evaluation of MLLMs, there is currently a lack of frameworks and relevant metrics. These frameworks and metrics are of significant importance in assessing MLLMs.


\subsection{Benchmarks for Multimodal Large Language Models}
MLLMs have demonstrated remarkable capabilities~\citep{llava,minigpt4,dai2023instructblip} and are poised to address increasingly complex multimodal tasks. Various benchmarks have emerged to evaluate MLLMs.
Some works focus on evaluating MLLMs using existing conventional multimodal datasets~\citep{wang2023visionllm} or only evaluate one or a few factors of MLLMs~\citep{shao2023tinylvlm,POPE,yu2023mmvet,bitton2023visitbench}, which may not provide a comprehensive evaluation suitable for these models.
Recent benchmarks~\citep{li2023seedbench,liu2023mmbench,fu2023mme} often focus on building a multimodal evaluation dataset for MLLMs. These benchmarks have been designed to transform open-ended predictions into predefined categorical choices. For instance, MME transforms free-form responses into binary True/False questions, while ~\citet{li2023seedbench,liu2023mmbench} employ multi-choice questions. However, the efficacy of these benchmarks is contingent upon the quality of the dataset construction and may suffer from scalability issues.
More recently, efforts such as ~\cite{yin2023lamm,xu2023lvlmehub} have attempted to establish evaluation frameworks, yet they have been characterized by limitations in terms of scalability and comprehensiveness. In response to these challenges, ChEF offers a standardized framework for conducting versatile evaluations and facilitates seamless integration of new models and tasks. 

==> sections/4.Framework.tex <==
\section{ChEF}
The design principles of ChEF are listed in Section~\ref{sec:design_principles}. The details of the four modules that constitute the framework are described in Section~\ref{sec:overview_chef}, based on which, the evaluations for the capabilities across six dinstint dimensions of desiderata are shown in Section~\ref{sec:desiderata}.
% 
% In this section, we will begin by introducing the design principles of the ChEF framework and providing an overview of the design details for the four modules that constitute this framework. We will then build upon this foundation by incorporating evaluations for the capabilities across six distinct dimensions of desiderata.

\subsection{Design Principles}
\label{sec:design_principles}


\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{sections/Figs/evaluation_pipeline_example.pdf}
    \caption{\textbf{Two examples of recipe in ChEF.} A recipe consists of \{\textit{scenario}, \textit{instruction}, \textit{inferencer}, \textit{metric}\}. The recipe of (a) is \{Flickr30k, ICE, PPL, Accuracy\}, while (b) is \{VOC2012, Query, Multiple Turns, mAP\}.}
  \label{fig:evaluation_pipeline_example}
  \vspace{-0.5cm}
\end{figure}


ChEF is a comprehensive evaluation framework aimed at providing a fair and holistic assessment of MLLMs' performance across diverse multimodal tasks, with the goal of accelerating research progress in the field of MLLMs. To accomplish this objective, our design principles encompass the following key aspects:

\textbf{1) Modularity:} As the field of MLLMs continues to advance rapidly, there is an increasing number of benchmark-related works, making it challenging to achieve unified evaluations within a single framework. Thus, we decouple the evaluation framework into four modular components: scenario, instruction, inferencer, and metric. This modular design enables flexible modification of each component and ensures consistent evaluation results across different benchmark datasets within the same framework.

\textbf{2) Scalability:} Within ChEF, we incorporate a diverse set of single-task and multiple-task datasets across our supported scenarios. Furthermore, we implement interfaces that streamline the process of integrating new scenarios into the framework. We actively encourage collaboration and contributions from the open-source community to expand the scope of scenarios available within ChEF.

\textbf{3) Flexibility:} We design ChEF to accommodate the varying input instruction formats supported by different MLLMs, including queries and in-context learning examples. By establishing fixed patterns for composing instructions using queries and in-context examples (ICE), we strive to encourage MLLMs to generate outputs that are suitable for the specific scenario. This flexibility enables the evaluation of MLLMs with diverse designs within a unified framework.

\textbf{4) Reliability:} We develope diverse inferencers for different scenarios within ChEF, which leverage MLLMs to generate predictions based on the provided instructions. The design of the inferencer module enhances the reliability of the evaluation results. Unlike directly evaluating the extracted information from MLLMs' output text, the scenario-specific inferencers are better tailored to reflect the precise perception or reasoning abilities that the scenario intends to assess. This optimization ensures greater reliability in the evaluation outcomes.

\textbf{5) Indicative:} Within ChEF, we utilize diverse metrics across different tasks. We assert that, for scenarios associated with traditional computer vision tasks, it is crucial to adapt and optimize the existing evaluation metrics to effectively assess MLLMs. By doing so, we ensure that our evaluation results serve as robust indicators of MLLMs' performance.


\subsection{Overview of ChEF}
\label{sec:overview_chef}

In order to adhere to the modularity principle of the framework, we divide ChEF into four main modular components: \textit{scenario}, \textit{instruction}, \textit{inferencer}, and \textit{metric}. The specific choices of the four components can be combined to form a recipe. For an illustration of the functionality and implementation approach of each module, we provide two examples of recipe in Figure~\ref{fig:evaluation_pipeline_example}. 

In Figure~\ref{fig:evaluation_pipeline_example} (a), the \textit{scenario} is Flickr30k, which is the test dataset to evaluate. The scenario, which pertains to the datasets and tasks utilized for evaluating the proficiency of MLLMs in visual and multi-modal tasks, is designed to be scalable for inclusion of any related dataset. 
% 
While traversing the scenario to evaluate a test sample,  top-$k$ ICE are retrieved from the dataset based on the image similarity. The selected ICE and the fo query serve as the \textit{instruction}. The instruction, which poses the MLLMs to generate response, contains different settings of query and ICE, for the flexibility of the evaluation.
% 
Following that, top-$k$ negative answers are retrieved from the scenario based on text similarity. These answers, alongside the correct answer, collectively constitute the answer pool, which is a limited text scope for MLLMs' response.
The ICE and each answer in the pool are fed into PPL, which serves as the \textit{inferencer}, for probability prediction, ultimately determining the final prediction from the answer pool. The inferencer, which pertains to how the model answers questions, includes multiple settings, for a relibale evaluation. 
% 
Finally, accuracy is employed as the \textit{metric} to determine the correctness of the predictions. Besides accuracy, the metric module contains severalwell-established metrics such as BLEU for caption tasks.

Similarly, the evaluation pipeline for the VOC2012 \textit{scenario} is presented In Figure~\ref{fig:evaluation_pipeline_example} (b), utilizing query for \textit{instruction}, multiple turns for \textit{inferencer}, and mAP as \textit{metric}. \footnote{Additional details within each module are presented in Supplementary Materials. }

The decoupled four modules enable support for distinct evaluation recipes, thereby facilitating diverse evaluation criteria. This modularity of ChEF allows for flexibility and adaptability to different evaluation requirements, providing evaluations across different benchmark datasets within the same framework.


\subsection{Desiderata}
\label{sec:desiderata}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{sections/Figs/recipe.pdf}
    \caption{\textbf{Recipes for evaluating six dimensions of desiderata.} All six dimensions are assessed on MMBench and ScienceQA, except for Hallucination, which is evaluated solely on MSCOCO. ICL evaluation uses random ICE, while others use standard queries.  Multiple turns inferencing is employed, with CoT and PPL utilized. For hallucination, a single PPL is employed. The metrics used for each dimension are specifically designed for their respective evaluations.  }
  \label{fig:recipes}
  \vspace{-0.3cm}
\end{figure}

As shown in Figure~\ref{fig:recipes}, building upon the ChEF framework, we implement evaluations based on six dimensions of desiderata. Each dimension is assessed using a specially designed recipe to ensure reliable evaluations. In assessing the desiderata, we place a stronger emphasis on evaluating the credibility, interactivity, and robustness of MLLMs as agents interacting with humans. We argue that MLLMs need to strengthen these abilities further to unlock new possibilities in the domain of multi-modal applications.

% Evaluating the quality of a model solely based on accuracy falls short of providing a holistic assessment. Metrics beyond accuracy, including reliability, interactivity, and robustness, also warrant consideration. Considering the aspects of coverage and social considerations, we have carefully selected following six vital metrics to gauge the model's performance:
\begin{figure}[htb]
    \centering
    \includegraphics[width=\textwidth]{sections/Figs/desiderata_examples.pdf}
    \caption{Give an example, we mark the distinguished design of each desiderata in red. Hallucination is solely evaluated on MSCOCO. For calibration evaluation, the prediction confidence is calculated to determine the gap between confidence and accuracy. Instruction Following is evaluated through verbalizer manipulation. In-context Learning is evaluated by providing ICE in the instruction. Robustness is assessed by introducing noise to both the image and text inputs. Language Performance is evaluated by instructing the model to generate chain-of-thought content. Hallucination is evaluated by querying whether a specific object is present in the image.
    % \textbf{Evaluation for each desiderata upon the example in (a).}
    }
  \label{fig:desiderata_examples}
  \vspace{-0.3cm}
\end{figure}

\textbf{Calibration} evaluates the model's accuracy and the appropriateness of its uncertainty, as highlighted by HELM~\citep{liang2022helm}. It is measured using the \textit{Expected Calibration Error} (ECE)~\citep{Pakdaman_Naeini_Cooper_Hauskrecht_2015,guo2017calibration}, which gauges the difference between the model’s predicted confidence, as shown in Figure~\ref{fig:desiderata_examples} and the actual probability the model is correct.

To estimate this difference with limited samples, the model's predictions are grouped into $m$ bins. Uniform-mass bins are used with $k=10$, ensuring an equal number of samples in each bin. Given a set of indices $i$ for samples in the $m$-th bin $\mathcal{B}m$, the average confidence and accuracy of $\mathcal{B}m$ are:
\begin{align}
&\operatorname{conf}\left(\mathcal{B}{m}\right)=\frac{1}{\left|\mathcal{B}{m}\right|}\sum_{i\in B_m}^{}\hat{p}i \
&\operatorname{Acc}\left(\mathcal{B}{m}\right)=\frac{1}{\left|\mathcal{B}{m}\right|}\sum{i\in \mathcal{B}m}^{}\mathbf{1}(\hat{y}i=y_i )
\end{align}
The ECE can then be approximated as:
\begin{equation}
\mathrm{ECE} =\sum_{m=1}^{k} \frac{\left|\mathcal{B}{m}\right|}{n}\left|\operatorname{conf}\left(\mathcal{B}{m}\right)-\operatorname{Acc}\left(\mathcal{B}{m}\right)\right|
\end{equation}
The gap between $\operatorname{conf}$ and $\operatorname{Acc}$ for a bin showcases the calibration discrepancy. A lower ECE implies a better-calibrated model, suggesting the predicted confidence aligns well with the true likelihood.

% \textbf{Calibration} aims to evaluate the model's performance to be simultaneously accurate and to provide appropriate uncertainty in its outputs, as emphasized in the work by HELM~\citep{liang2022helm}. An example is showed in Figure ~\ref{fig:desiderata_examples}. This is particularly significant in risk scenarios  We evaluate calibration by \textit{Expected Calibration Error} (ECE)~\citep{Pakdaman_Naeini_Cooper_Hauskrecht_2015,guo2017calibration}. Formally, let $y$ be ground truth, and $\hat{y}$ be model's prediction with associated confidence $\hat{p}$. The ECE examines the
% difference between the model’s predicted confidence $\hat{p}$ and the probability the model is correct given $\hat{p}$, as shown in equation~\ref{equ:calibration_1}.
% \begin{equation}
%     \mathrm{ECE}=\mathbb{E}  [| \hat{p}-\mathbb{E} (y=\hat{y}|\hat{p} )| ] 
%     \label{equ:calibration_1} 
% \end{equation}
% To estimate the expected accuracy $\mathbb{E} (y=\hat{y}|\hat{p} )$ from finite samples, we compute the ECE by binning the model’s predictions into $m$ bins following prior work~\citep{guo2017calibration,liang2022helm}. We choose uniform-mass bins for better approximation with $k=10$, where an equal number of samples fall into each bin. Let $\mathcal{B}_m$ be a set of indices $i$ of samples falling in $m$-th bin, then the average confidence and accuracy of $\mathcal{B}_m$ are defined as 
% \begin{align}
% &\operatorname{conf}\left(\mathcal{B}_{m}\right)=\frac{1}{\left|\mathcal{B}_{m}\right|}\sum_{i\in B_m}^{}\hat{p}_i  \label{equ:calibration_2} \\
% &\operatorname{Acc}\left(\mathcal{B}_{m}\right)=\frac{1}{\left|\mathcal{B}_{m}\right|}\sum_{i\in \mathcal{B}_m}^{}\mathbf{1}(\hat{y}_i=y_i )  \label{equ:calibration_3} 
% \end{align}
% Therefore, we can approximates equation ~\ref{equ:calibration_1} by equation~\ref{equ:calibration_4}.
% \begin{equation}
% \mathrm{ECE} =\sum_{m=1}^{k} \frac{\left|\mathcal{B}_{m}\right|}{n}\left|\operatorname{conf}\left(\mathcal{B}_{m}\right)-\operatorname{Acc}\left(\mathcal{B}_{m}\right)\right|
% \label{equ:calibration_4}
% \end{equation}
% The difference between $\operatorname{conf}$ and $\operatorname{Acc}$ for a given bin represents the calibration gap(visualization in Figure~\ref{fig:calibration} ). The lower the ECE, the better the calibration of the model, indicating that the predicted confidence $\hat{p}$ more accurately represents the true probability. 

\textbf{In-context Learning} \label{sec:icl}
aims to evaluate ICL capability, enabling models to perform tasks without gradient-based training. Such capability can generalize to new scenarios, representing potential technological advances. While LLMs have shown ICL ability, most MLLMs lack it, making ICL evaluation crucial for MLLMs.
ICL utilizes a few ICE before a query to improve LLMs' performance. For multimodal tasks involving visual data, integrating the ICE with images is logical. However, some MLLMs only support single-image input, restricting ICE's image inclusion. Given these constraints, we implement two ICL approaches: one without images and another with them.

To assess ICL capability, we use ICE for specific scenarios and compute accuracy, then determine the relative accuracy change as the final score. Considering potential biases in multiple-choice questions, we introduce the \textit{Relative ICL Accuracy for Multiple-choice} (RIAM) to better evaluate ICL. RIAM measures the accuracy change beyond random guessing:

\begin{equation}
\mathrm{RIAM} = \frac{\operatorname{Acc}_{icl}-\operatorname{Acc}_{basic}}{\operatorname{Acc}_{basic}-\operatorname{Acc}_{random}}
\label{equ:icl}
\end{equation}

where $\operatorname{Acc}_{basic}$ denotes the accuracy in the 0-shot setting, $\operatorname{Acc}_{icl}$ represents the average accuracy values for varying numbers of ICE, $\operatorname{Acc}_{random}$ represents the accuracy of random guessing.

% \textbf{In-context Learning} \label{sec:icl}
% aims to evaluate the capability of in-context learning(ICL), which enables models to perform new tasks without any gradient-based training~\citep{wu2023openicl, brown2020language}.This ability is capable of generalizing to unseen cases, which opens up many new technological possibilities that were previously considered unique to humans. While in the field of NLP, LLMs have demonstrated ICL capabilities, within the domain of MLLMs, this ability remains unexplored. Most MLLMs lack ICL capabilities~\cite{li2023otter}. Therefore, considering ICL capability as a dimension in the evaluation of multimodal large models is crucial. 

% ICL adds a small number of ICE before query as the instruction and has demonstrated its capability to enhance the performance of LLMs in few-shot scenarios. Given that multimodal tasks typically involve visual data, incorporating the ICE with image in MLLMs is a reasonable approach. However, some MLLMs currently only support single-image input, and there is already an image in the query, which prevents the inclusion of ICE's image. Considering the limited support for multi-image input in certain MLLMs, we have implemented two ICL methodologies: one utilizing ICE without image and the other incorporating ICE with images. An example of ICE with images is shown in Figure~\ref{fig:desiderata_examples}. For the selection of ICE, we have implemented retriever methods such as Random, Fixed and Top-$k$, as mentioned in Section~\ref{sec:Instruction}.

% To measure the model's ICL capability, we utilize ICE as instruction for each specific scenario and compute their accuracy, and use the relative accuracy change as the final score, Specifically, we compute the accuracy under the 0-shot setting (without using ICE) and the average accuracy values for varying numbers of ICE, ranging from $1$ to $N$. In multiple-choice questions, random guessing can yield an expected lower-bound accuracy, which can be misleading in terms of performance evaluation. To mitigate the impact of this potentially deceptive performance on robustness assessments, we systematically eliminate the bias introduced by random choice. Therefore, we introduce the \textit{Relative ICL Accuracy for Multiple-choice} (RIAM), adapted from \citet{chen2023benchmarking, schiappa2023robustness}, to more accurately assess the model's ICL capability. The RIAM primarily calculates the relative accuracy change of the model beyond random guessing accuracy before and after using ICE, as depicted in Equation~\ref{equ:icl},


% \begin{equation}
% \mathrm{RIAM} = \frac{\operatorname{acc}_{icl}-\operatorname{acc}_{random}}{\operatorname{acc}_{basic}-\operatorname{acc}_{random}} \times 50 +50
% \label{equ:icl}
% \end{equation}
% where $acc_{basic}$ denotes the accuracy in the 0-shot setting, $acc_{icl}$ represents the average accuracy values for varying numbers of ICE, $\operatorname{acc}_{random}$ represents the accuracy of random guessing.

\textbf{Instruction Following}
We use three categories of instructions for verbalizer manipulation: \textit{natural, neutral, unnatural}~\citep{li2023instructionfollowing}, to assess how effectively models follow varying instructions. The alignment with prior knowledge ranks as \textit{natural} $>$ \textit{neutral} $>$ \textit{unnatural}. In \textit{natural} instructions, familiar verbalizers align with common knowledge (e.g., “1\textbar2\textbar3\textbar4” for “A\textbar B\textbar C\textbar D”). \textit{Neutral} instructions use unrelated verbalizers, while \textit{unnatural} instructions shift verbalizers, causing a mismatch.

To measure adherence to these instructions, we compute the \textit{match ratio} (MR), signifying the percentage of samples aligned with the verbalizer instructions. A higher MR demonstrates the model's proficiency in instruction following.



% \textbf{Instruction Following} 
% Taking inspiration from \citep{li2023instructionfollowing}, we utilize three groups of instructions for verbalizer manipulation: \textit{natural, neutral, unnatural}, to evaluate how well models can follow instructions that may not align with their priors. The levels in terms of aligning with
% prior knowledge of these three groups are ranked as \textit{natural} $>$ \textit{neutral} $>$ \textit{unnatural}. We expect the model to answer the question following instructions and generate a new answer corresponding to the original answer. In \textit{natural} instructions, we choose multiple verbalizers that align with prior knowledge (e.g. “1\textbar2\textbar3\textbar4” or “I\textbar II\textbar III\textbar IV” corresponding to “A\textbar B\textbar C\textbar D”). In \textit{neutral} instructions, we select multiple verbalizers that are semantically irrelevant to given chioce(e.g. “Smith\textbar Johnson\textbar Williams\textbar Jones” corresponding to “A\textbar B\textbar C\textbar D"). In \textit{unnatural} instructions, verbalizers are shifted to their next choice in original choices and contradict with prior knowledge(e.g. “D\textbar A\textbar B\textbar C" corresponding to “A\textbar B\textbar C\textbar D").  These instructions are employed to elicit specific responses from the model, as illustrated in Figure~\ref{fig:desiderata_examples}. 
% We calculate the \textit{match ratio} (MR) to determine the percentage of samples that adhere to the verbalizer manipulation instructions, mapping their original answers to corresponding new answers. This calculation helps mitigate the influence of the model's accuracy in answering questions and highlights its proficiency in following verbalizer manipulation instructions. A higher MR indicates a superior ability of the model to follow instructions. 
 
\textbf{Language Performance}
Evaluating the quality of language generation poses challenges, often requiring multifaceted scoring. GPT metrics have recently shown to correlate well with human evaluations compared to traditional methods~\citep{zheng2023judging,liu2023geval,wang2023chatgpt}. Hence, we use GPT to assess the chain-of-thought output of models in the VQA scenario, as depicted in Figure~\ref{fig:desiderata_examples}.

However, VQA evaluations present unique challenges due to GPT's inability to access visual data. To address this, several adaptations for GPT's multimodal task evaluations have been made. First, GPT is provided with ground truth answers, ensuring that the generated content remains faithful to the original thought. Additionally, GPT assumes that any visual details in model responses are present in the image, which helps in avoiding misjudgments about image descriptions.
Moreover, the evaluation only considers samples with accurate conclusions from the test model, minimizing the influence of conclusion accuracy on the assessment of language quality. Instead of pairwise comparisons, we employ the efficient \textit{Single Answer Grading} approach~\citep{zheng2023judging}, which aligns well with human expert opinions. Lastly, we utilize \textit{Multiple Evidence Calibration}~\citep{wang2023large}, to enhance the GPT scoring reliability. We prompt GPT to produce explanations before settling on a final score. By using autoregressive models, GPT can calibrate scores based on these evaluations. We further refine this by averaging scores from multiple GPT responses for each evaluation query, ensuring more accurate and consistent results.

% \textbf{Language performance}
% Evaluating the quality of natural language generation is a challenging task, often requiring scoring based on various aspects such as coherence, consistency, fluency, and more. Recent studies~\citep{zheng2023judging,liu2023geval,wang2023chatgpt} have indicated that GPT metrics typically exhibit superior performance compared to traditional reference-based and reference-free baseline metrics in terms of their correlation with human quality judgments. Thus, We employ GPT to score the chain-of-thought text generated by the model in the VQA scenario, as shown in Figure~\ref{fig:desiderata_examples}, aiming to evaluate the model's language performance.

% In contrast to NLP, where GPT can evaluate the quality of natural language generation without references~\citep{zheng2023judging,liu2023geval,wang2023chatgpt}, the evaluation process in VQA scenario presents a distinct challenge as GPT lacks access to visual information. Therefore, we have implemented specific adaptations for evaluating GPT's performance in multimodal tasks: 

% \textbf{1) Reference-Based Evaluation:} we provide GPT with ground truth answers as reference during the evaluation,  which ensures faithfulness of the chain of thought.

% \textbf{2) Visual Information Assumption:} GPT is prompted to assume that all visual information mentioned in the test model's responses is contained in the image. This measure prevents GPT from misjudging descriptions of image in the chain of thought as language hallucinations(which may not be explicitly stated in the query text). This helps avoid unwarranted reductions in the language performance score.

% \textbf{3) Selective Sampling of Correct Conclusions:} We selectively extract samples in which the test model's conclusions are correct. This reduces the impact of conclusion accuracy on the evaluation of language generation quality. 

% \textbf{4) Efficient and Scalable Evaluation}: For more efficient and scalable evaluation, instead of pairwise comparisons, we individually assess each model's response, which called \textit{Single Answer Grading},as demonstrated in ~\citep{zheng2023judging}, exhibits high agreement with human experts.

% \textbf{5) Multiple Evidence Calibration~\citep{wang2023large}:} In order to make the GPT score more reliable and interpretable, we prompt the GPT to generate explanation as evaluation evidence before generating the final overall score. Thanks to the properties of autoregressive models, this method allows GPT to calibrate scores based on evaluation evidence. In order to further reduce the systematic error of GPT evaluation, we conducted multiple evidence calibration, sampling multiple GPT responses for each evaluation query, and taking the average score of all responses as the final evaluation score.

\textbf{Robustness} describes an MLLM's ability to provide accurate and meaningful outputs despite diverse challenges in input data. This quality ensures the model's trustworthiness for real-world applications, especially when faced with data corruption and variations, as visualized in Figure~\ref{fig:desiderata_examples}. Drawing from recent studies~\citep{liang2022helm,qiu2022multimodal,chen2023benchmarking,schiappa2023robustness}, we introduce select image and text corruptions to evaluate our model's robustness.

For images, we adopte corruption categories like \textit{noise, blur, weather, digital}~\citep{DBLP:journals/corr/abs-1903-12261}, and \textit{others}—the last category encompassing basic data augmentation techniques. Textual corruption, in turn, is divided into categories of \textit{basic, sentence, word, character}~\citep{chen2023benchmarking}, and \textit{choice}, with the \textit{choice} category being especially tailored for multiple-choice questions. To emulate real-world scenarios, we intertwine five sets of these corruption types with their severity levels for both images and texts. This hybrid approach lets us assess how the model grapples with combined disruptions in both domains.
\begin{equation} % @wangzhipin
\mathrm{RRM} = \frac{\operatorname{Acc_{crp}}-\operatorname{Acc_{random}}}{\operatorname{Acc}-\operatorname{Acc_{random}}}
\label{equ:rob_match}
\end{equation}

Furthermore, to gain a deeper understanding of our model's robustness, we use the \textit{Relative Robustness for Multiple-choice} (RRM), which calculates the model's relative accuracy alteration, beyond mere random guessing, pre and post-corruption. This is encapsulated in Equation~\ref{equ:rob_match}, where $\operatorname{Acc}$ and $\operatorname{Acc_{crp}}$ denote accuracy metrics before and after the corruptions, while $\operatorname{Acc_{random}}$ indicates the benchmark accuracy from random guessing.



% \textbf{Robustness} refers to the capability of MLLMs to maintain accurate performance and meaningful outputs in the face of diverse challenges and variations in input data. This includes addressing data corruption and perturbations, which ensures the model's reliability in real-world applications, as illustrated in Figure ~\ref{fig:desiderata_examples}. To evaluate the robustness of our model, we have carefully selected mild image and text corruptions, drawing inspiration from recent work~\citep{liang2022helm,qiu2022multimodal,chen2023benchmarking,schiappa2023robustness}.

% For image corruptions, we incorporated five corruption categories: \textit{noise, blur, weather, and digital} (sourced from ImageNet-C~\citep{DBLP:journals/corr/abs-1903-12261}), and \textit{other}, which includes fundamental data augmentation techniques. For text corruption, we introduce five categories like ~\citep{chen2023benchmarking}: \textit{basic, sentence, word, character,} and \textit{choice}. The \textit{choice} category specifically represents additional corruption introduced for multiple-choice questions. To simulate real-world complexity, we have randomly combined five sets of corruption types and their corresponding severity levels for both visual and textual inputs. This allows us to test the model's performance in handling joint corruptions across visual and textual domains, mimicking the complexities found in real-world scenarios. 

% To more accurately assess the model's robustness, we introduce the \textit{Relative Robustness for Multiple-choice} (RRM) as described in section \ref{sec:icl}, The RRM primarily calculates the relative accuracy change of the model beyond random guessing accuracy before and after corruptions, as depicted in Equation~\ref{equ:rob_match}.
% \begin{equation} % @wangzhipin
% \mathrm{RRM \%} = \frac{\operatorname{Acc_{crp}}-\operatorname{Acc_{random}}}{\operatorname{Acc}-\operatorname{Acc_{random}}} \times 100\%
% \label{equ:rob_match}
% \end{equation}
% where $\operatorname{Acc}$ and $\operatorname{Acc_{crp}}$ represents the accuracy before and after corruptions respectively, and $\operatorname{Acc_{random}}$ represents the accuracy of random guessing.

\textbf{Hallucination} pertains to the content generated that strays from or doesn't align with the source material~\citep{Ji_2023}. MLLMs, akin to LLMs, grapple with this issue, particularly when it comes to object hallucination, where generated descriptions for an image might introduce objects that aren't present in the actual image~\citep{9706727}. To assess this, we utilize the Polling-based Object Probing Evaluation (POPE)~\citep{POPE} on MSCOCO. This method transforms hallucination evaluation into a set of binary classification tasks. Essentially, the MLLM is posed direct Yes-or-No questions about the existence of particular objects in the images, like `Is there a car in the image?', as depicted in Figure~\ref{fig:desiderata_examples}.

For deriving these probing objects, three polling strategies by POPE are used: random sampling, sampling based on object popularity, and based on frequently co-occurring objects. Alongside, we employ PPL to fortify our assessment's trustworthiness. Metrics like accuracy, precision, recall, F1-Score, and the proportion of “Yes" responses serve as the cornerstone of our evaluation.

% \textbf{Hallucination} refers to the generated content that is nonsensical or unfaithful to the provided source content~\citep{Ji_2023}. Similar to LLMs, MLLMs also encounter the challenge of hallucination. Since objects are the core elements
% that contribute to the visual semantics of an image, we study the object hallucination problem, which refers that the generated descriptions for a given image containing objects that are inconsistent with the image~\citep{9706727}. As a result, we utilize the Polling-based Object Probing Evaluation (POPE) pipeline~\citep{POPE} on the MSCOCO dataset~\citep{mscoco}. The fundamental concept behind this approach is to transform the evaluation of hallucination into a series of binary classification tasks. This is achieved by presenting MLLM with straightforward Yes-or-No questions regarding the presence of specific objects within the images (e.g., “Is there a car in the image?"), as illustrated in Figure ~\ref{fig:desiderata_examples}. Each image is prompted with six such Yes-or-No questions. 
% To generate the probing objects, POPE consider three polling strategies by sampling the objects randomly, from popular objects, and among those frequently co-occurring objects, respectively. Additionally, we employ PPL to enhance the reliability of our evaluation. Similar to POPE, we also calculate evaluation metrics such as accuracy, precision, recall, F1-Score, and the ratio of “Yes" responses.

==> submission/math.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

